Lectures on Scattering Amplitudes in String Theory

In these lecture notes, we take a closer look at the calculation of scattering amplitudes for the bosonic string. It is believed that string theories form the UV completions of (super)gravity theories. Support for this claim can be found in the (on-shell) scattering amplitudes of strings. On the other hand, studying these string scattering amplitudes opens a window on the UV behavior of the string theories themselves. In these short set of lectures, we discuss the two-dimensional Polyakov path integral for the string, and its gauge symmetries, the connection to Riemann surfaces and how to obtain some of the simplest string scattering amplitudes. We end with some comments on more advanced topics. For simplicity we limit ourselves to bosonic open string theory in 26 dimensions.

==> Bibliography.tex <==
\chapter{Bibliography per chapter}
\section{Chapter \ref{BWc:Riemann}}
\begin{itemize}
\item The first section \ref{BWs:WSasRS} is based
on:\cite{Hitchin:2004b3c}, \cite{Nakahara:2003nw},
\cite{Polchinski:1998rq}, \cite{Olson:200un}, \cite{Lee:1997};
\item The second section \ref{BWs:RiemannSurfaces} is based on:
\cite{Olson:200un}, \cite{Nakahara:2003nw}, \cite{Farkas:1980},
\cite{Miranda:1995};
\item The third section \ref{BWs:PropRS} is based
on:\cite{Olson:200un}, \cite{Nakahara:2003nw}, \cite{Farkas:1980},
\cite{Miranda:1995}, \cite{D'Hoker:1988ta}.
\end{itemize}


\section{Chapter \ref{BWc:Fixing}}
\section{Chapter \ref{BWc:Amplitudes}}
First section \ref{BWs:AmplitudesGenFunct} is based heavily on
Polchinski, chapter 6.2 and Nakahara \cite{Nakahara:2003nw}, 14.2.
Also inspiration in D'Hoker and Phong (1988) \cite{D'Hoker:1988ta}
2.B.


\begin{itemize}
 \item Chapter \ref{BWc:Fixing}
\item Chapter \ref{BWc:Amplitudes}. First section \ref{BWs:AmplitudesGenFunct} is based heavily on Polchinski, chapter 6.2 and Nakahara \cite{Nakahara:2003nw}, 14.2. Also inspiration in D'Hoker and Phong (1988) \cite{D'Hoker:1988ta} 2.B.
\end{itemize}

